Building a Fine-Grained Entity Typing System Overnight for a New X (X = Language, Domain, Genre)

Recent research has shown great progress on fine-grained entity typing. Most existing methods require pre-defining a set of types and training a multi-class classifier from a large labeled data set based on multi-level linguistic features. They are thus limited to certain domains, genres and languages. In this paper, we propose a novel unsupervised entity typing framework by combining symbolic and distributional semantics. We start from learning general embeddings for each entity mention, compose the embeddings of specific contexts using linguistic structures, link the mention to knowledge bases and learn its related knowledge representations. Then we develop a novel joint hierarchical clustering and linking algorithm to type all mentions using these representations. This framework doesn't rely on any annotated data, predefined typing schema, or hand-crafted features, therefore it can be quickly adapted to a new domain, genre and language. Furthermore, it has great flexibility at incorporating linguistic structures (e.g., Abstract Meaning Representation (AMR), dependency relations) to improve specific context representation. Experiments on genres (news and discussion forum) show comparable performance with state-of-the-art supervised typing systems trained from a large amount of labeled data. Results on various languages (English, Chinese, Japanese, Hausa, and Yoruba) and domains (general and biomedical) demonstrate the portability of our framework.

==> 3.5entityLinking.tex <==
\subsection{Entity Linking}
\label{sec:entityLinking}
%\todo{in section 3.2: explain the story: we need to compose embeddings for specific contexts, but we cannot use all neighbor contexts}
%\todo{explain why you design these meta-paths, why distinguish directions, why throw away other dependency types}

%Based on these hypotheses, 
%We will present how to type concepts step by step.
%\input{3.1conceptidentification}
%\todo{write more details}
%As described in Section 3.1, 

%Next we will link each mention to existing KBs to determine its knowledge representation and extract the type path. 
We utilize a domain and language independent entity linking (EL) system~\cite{Wang2015} to link each mention to existing KBs to determine its knowledge representation and extract the type path. This system is based on an unsupervised collective inference approach. 

%and thus is domain and language independent. 
%The overall framework is shown in Figure~\ref{entityLinking}. 

%\begin{figure}[!htp]%{R}{0.9\textwidth} 
%\centering
%% \includegraphics[width=1.\textwidth]{Figures/generalEmbedding1.eps}
%\includegraphics[width=.45\textwidth]{Figures/el.pdf}
%\caption{Entity Linking System Overview}
%\label{entityLinking}
%\end{figure} d

Given a set of entity mentions $M = \{m_1, m_2, ..., m_n\}$, this system first constructs a graph for all entity mentions based on their co-occurrence within a paragraph, which, in our experiment, is taken to mean `five continuous sentences.' Then, for each entity mention $m$, this system uses the surface form dictionary $<f, {e_1, e_2, ..., e_k}>$, where ${e_1, e_2, ..., e_k}$ is the set of entities with surface form $f$ according to their properties (e.g., labels, names, aliases), to locate a list of candidate entities $e \in E$ and compute the importance score by an entropy based approach~\cite{Zheng2014}. Finally, it computes similarity scores for each entity mention and candidate entity pair $<m, e>$ and selects the candidate with the highest score as the appropriate entity for linking. We select highly linkable mentions (confidence score $>0.95$) and their corresponding type paths for next steps. In our experiments, about $77.7\%$ entity mentions in the general news domain and about $71.4\%$ percent in the biomedical domain can be linked to KBs with high confidence.%In our experiment, we assume the linking result is confident when the highest score $>0.95$. This system doesn't rely on any deep linguistic analysis on the source documents, so it can be easily adapted to new genres, domains or languages. 

%Compared with state-of-the-art supervised EL method, it can significantly get at least 9 absolute gain in linking accuracy for both general domain and biomedical domain.

%We applied this system to link each entity mention to knowledge bases (e.g., YAGO for general domain, and BioPortal for biomedical domain) and select highly linkable entity mentions and their corresponding type paths. %Considering the examples in Section 1 again, we can link the entity mention ``\textbf{Mitt Romney}'' to YAGO and extract a type path from the entity title to the root: '\emph{Mitt Romney}', '\emph{Governor}', '\emph{Politician}', '\emph{Leader}', '\emph{Person}', '\emph{Entity}'. Similarly, we can link ``\textbf{RAS}'' to ``\emph{Proto-Oncogene Proteins p21(ras)}'' in BioPortal and extract the type name path from the entity to the root of an ontology as: '\emph{Proto-Oncogene Proteins p21(ras)}', '\emph{Proto-Oncogene Proteins}', '\emph{Oncogene Proteins}', '\emph{Neoplasm Proteins}', '\emph{Proteins}', '\emph{Amino Acids, Peptides, and Proteins}', '\emph{Chemicals and Drugs (MeSH Category)}', '\emph{Topical Descriptor}', '\emph{MeSH Descriptors}'. In our experiments, about $77.7\%$ entity mentions in general news domain and about $71.4\%$ percent in biomedical domain can be linked to KBs with high confidence.
